Learning based E2E Energy Efficient in Joint Radio and NFV Resource Allocation for 5G and Beyond Networks

In this paper, we propose a joint radio and core resource allocation framework for NFV-enabled networks. In the proposed system model, the goal is to maximize energy efficiency (EE), by guaranteeing end-to-end (E2E) quality of service (QoS) for different service types. To this end, we formulate an optimization problem in which power and spectrum resources are allocated in the radio part. In the core part, the chaining, placement, and scheduling of functions are performed to ensure the QoS of all users. This joint optimization problem is modeled as a Markov decision process (MDP), considering time-varying characteristics of the available resources and wireless channels. A soft actor-critic deep reinforcement learning (SAC-DRL) algorithm based on the maximum entropy framework is subsequently utilized to solve the above MDP. Numerical results reveal that the proposed joint approach based on the SAC-DRL algorithm could significantly reduce energy consumption compared to the case in which R-RA and NFV-RA problems are optimized separately.

==> citation_E2E-RA.bbl.tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{8320765}
I.~{Afolabi}, T.~{Taleb}, K.~{Samdanis}, A.~{Ksentini}, and H.~{Flinck},
  ``Network slicing and softwarization: A survey on principles, enabling
  technologies, and solutions,'' \emph{IEEE Communications Surveys Tutorials},
  vol.~20, no.~3, pp. 2429--2453, Mar. 2018.

\bibitem{8125672}
Z.~{Chang}, Z.~{Zhou}, S.~{Zhou}, T.~{Chen}, and T.~{Ristaniemi}, ``Towards
  service-oriented {5G}: Virtualizing the networks for
  everything-as-a-service,'' \emph{IEEE Access}, vol.~6, pp. 1480--1489, Dec.
  2018.

\bibitem{mijumbi2015design}
R.~{Mijumbi}, J.~{Serrat}, J.~{Gorricho}, N.~{Bouten}, F.~{De Turck}, and
  S.~{Davy}, ``Design and evaluation of algorithms for mapping and scheduling
  of virtual network functions,'' in \emph{Proc. IEEE Conference on Network
  Softwarization (NetSoft)}, Apr. 2015, pp. 1--9.

\bibitem{mijumbi2016network}
R.~{Mijumbi}, J.~{Serrat}, J.~{Gorricho}, N.~{Bouten}, F.~{De Turck}, and
  R.~{Boutaba}, ``Network function virtualization: {State}-of-the-art and
  research challenges,'' \emph{IEEE Communications Surveys Tutorials}, vol.~18,
  no.~1, pp. 236--262, Sep. 2016.

\bibitem{herrera2016resource}
J.~{Gil Herrera} and J.~F. {Botero}, ``Resource allocation in{ NFV: A}
  comprehensive survey,'' \emph{IEEE Transactions on Network and Service
  Management}, vol.~13, no.~3, pp. 518--532, Sep. 2016.

\bibitem{8675284}
A.~N. {Al-Quzweeni}, A.~Q. {Lawey}, T.~E.~H. {Elgorashi}, and J.~M.~H.
  {Elmirghani}, ``Optimized energy aware {5G} network function
  virtualization,'' \emph{IEEE Access}, vol.~7, pp. 44\,939--44\,958, Mar.
  2019.

\bibitem{riera2014virtual}
J.~F. {Riera}, E.~{Escalona}, J.~{Batallé}, E.~{Grasa}, and J.~A.
  {García-Espín}, ``Virtual network function scheduling: {Concept} and
  challenges,'' in \emph{Proc. 2014 International Conference on Smart
  Communications in Network Technologies (SaCoNeT)}, June 2014, pp. 1--5.

\bibitem{alliance2016description}
N.~Alliance, ``Description of network slicing concept,'' \emph{NGMN 5G P},
  vol.~1, p.~1, Jan. 2016.

\bibitem{7926921}
J.~{Ordonez-Lucena}, P.~{Ameigeiras}, D.~{Lopez}, J.~J. {Ramos-Munoz},
  J.~{Lorca}, and J.~{Folgueira}, ``Network slicing for 5{G} with {SDN}/{NFV}:
  Concepts, architectures, and challenges,'' \emph{IEEE Communications
  Magazine}, vol.~55, no.~5, pp. 80--87, May. 2017.

\bibitem{7243304}
R.~{Mijumbi}, J.~{Serrat}, J.~{Gorricho}, N.~{Bouten}, F.~{De Turck}, and
  R.~{Boutaba}, ``Network function virtualization: State-of-the-art and
  research challenges,'' \emph{IEEE Communications Surveys Tutorials}, vol.~18,
  no.~1, pp. 236--262, Sep. 2016.

\bibitem{7945848}
M.~{Mechtri}, C.~{Ghribi}, O.~{Soualah}, and D.~{Zeghlache}, ``{NFV}
  orchestration framework addressing {SFC} challenges,'' \emph{IEEE
  Communications Magazine}, vol.~55, no.~6, pp. 16--23, Jun. 2017.

\bibitem{hossain20155g}
E.~{Hossain} and M.~{Hasan}, ``{5G} cellular: key enabling technologies and
  research challenges,'' \emph{IEEE Instrumentation Measurement Magazine},
  vol.~18, no.~3, pp. 11--21, June 2015.

\bibitem{7143328}
H.~{Dahrouj}, A.~{Douik}, O.~{Dhifallah}, T.~Y. {Al-Naffouri}, and
  M.~{Alouini}, ``Resource allocation in heterogeneous cloud radio access
  networks: advances and challenges,'' \emph{IEEE Wireless Communications},
  vol.~22, no.~3, pp. 66--73, June 2015.

\bibitem{8715830}
P.~{Chemouil}, P.~{Hui}, W.~{Kellerer}, Y.~{Li}, R.~{Stadler}, D.~{Tao},
  Y.~{Wen}, and Y.~{Zhang}, ``Special issue on artificial intelligence and
  machine learning for networking and communications,'' \emph{IEEE Journal on
  Selected Areas in Communications}, vol.~37, no.~6, pp. 1185--1191, 2019.

\bibitem{8932445}
J.~{Pei}, P.~{Hong}, M.~{Pan}, J.~{Liu}, and J.~{Zhou}, ``Optimal {VNF}
  placement via deep reinforcement learning in {SDN/NFV}-enabled networks,''
  \emph{IEEE Journal on Selected Areas in Communications}, vol.~38, no.~2, pp.
  263--278, 2020.

\bibitem{8354944}
A.~{Martin}, J.~{Egaña}, J.~{Flórez}, J.~{Montalbán}, I.~G. {Olaizola},
  M.~{Quartulli}, R.~{Viola}, and M.~{Zorrilla}, ``Network resource allocation
  system for {QoE}-aware delivery of media services in {5G} networks,''
  \emph{IEEE Transactions on Broadcasting}, vol.~64, no.~2, pp. 561--574, 2018.

\bibitem{xie2016service}
Y.~Xie, Z.~Liu, S.~Wang, and Y.~Wang, ``Service function chaining resource
  allocation: A survey,'' \emph{arXiv preprint arXiv:1608.00095}, 2016.

\bibitem{8480442}
M.~M. {Tajiki}, S.~{Salsano}, L.~{Chiaraviglio}, M.~{Shojafar}, and
  B.~{Akbari}, ``Joint energy efficient and {QoS}-aware path allocation and
  {VNF} placement for service function chaining,'' \emph{IEEE Transactions on
  Network and Service Management}, vol.~16, no.~1, pp. 374--388, 2019.

\bibitem{7417401}
M.~T. {Beck} and J.~F. {Botero}, ``Coordinated allocation of service function
  chains,'' in \emph{Proc IEEE Global Communications Conference (GLOBECOM)},
  San Diego, CA, USA, Dec. 2015, pp. 1--6.

\bibitem{8170213}
H.~{Li}, L.~{Wang}, X.~{Wen}, Z.~{Lu}, and L.~{Ma}, ``Constructing service
  function chain test database: An optimal modeling approach for coordinated
  resource allocation,'' \emph{IEEE Access}, vol.~6, pp. 17\,595--17\,605,
  2018.

\bibitem{liu2017dynamic}
J.~{Liu}, W.~{Lu}, F.~{Zhou}, P.~{Lu}, and Z.~{Zhu}, ``On dynamic service
  function chain deployment and readjustment,'' \emph{IEEE Transactions on
  Network and Service Management}, vol.~14, no.~3, pp. 543--553, Sep. 2017.

\bibitem{81702199999}
J.~{Pei}, P.~{Hong}, K.~{Xue}, D.~{Li}, D.~S.~L. {Wei}, and F.~{Wu},
  ``Two-phase virtual network function selection and chaining algorithm based
  on deep learning in {SDN/NFV}-enabled networks,'' \emph{IEEE Journal on
  Selected Areas in Communications}, vol.~38, no.~6, pp. 1102--1117, 2020.

\bibitem{riggio2016scheduling}
R.~{Riggio}, A.~{Bradai}, D.~{Harutyunyan}, T.~{Rasheed}, and T.~{Ahmed},
  ``Scheduling wireless virtual networks functions,'' \emph{IEEE Transactions
  on Network and Service Management}, vol.~13, no.~2, pp. 240--252, June 2016.

\bibitem{cohen2015near}
R.~{Cohen}, L.~{Lewin-Eytan}, J.~S. {Naor}, and D.~{Raz}, ``Near optimal
  placement of virtual network functions,'' in \emph{Proc. IEEE Conference on
  Computer Communications (INFOCOM)}, 2015, pp. 1346--1354. Kowloon, Hong Kong.
  Apr.

\bibitem{8611305}
S.~{Agarwal}, F.~{Malandrino}, C.~F. {Chiasserini}, and S.~{De}, ``{VNF}
  placement and resource allocation for the support of vertical services in
  {5G} networks,'' \emph{IEEE/ACM Transactions on Networking}, vol.~27, no.~1,
  pp. 433--446, 2019.

\bibitem{8255993}
A.~{Alleg}, T.~{Ahmed}, M.~{Mosbah}, R.~{Riggio}, and R.~{Boutaba},
  ``Delay-aware {VNF} placement and chaining based on a flexible resource
  allocation approach,'' in \emph{2017 13th International Conference on Network
  and Service Management (CNSM)}, 2017, pp. 1--7.

\bibitem{cao2017vnf}
J.~Cao, Y.~Zhang, W.~An, X.~Chen, J.~Sun, and Y.~Han, ``{VNF-FG} design and
  {VNF} placement for {5G} mobile networks,'' \emph{Science China Information
  Sciences}, vol.~60, no.~4, p. 040302, 2017.

\bibitem{8316876}
M.~{Dieye}, S.~{Ahvar}, J.~{Sahoo}, E.~{Ahvar}, R.~{Glitho}, H.~{Elbiaze}, and
  N.~{Crespi}, ``{CPVNF}: Cost-efficient proactive {VNF} placement and chaining
  for value-added services in content delivery networks,'' \emph{IEEE
  Transactions on Network and Service Management}, vol.~15, no.~2, pp.
  774--786, 2018.

\bibitem{8424410}
L.~{Tang}, H.~{Yang}, R.~{Ma}, L.~{Hu}, W.~{Wang}, and Q.~{Chen}, ``Queue-aware
  dynamic placement of virtual network functions in {5G} access network,''
  \emph{IEEE Access}, vol.~6, pp. 44\,291--44\,305, 2018.

\bibitem{8281644}
D.~{Li}, P.~{Hong}, K.~{Xue}, and j.~{Pei}, ``Virtual network function
  placement considering resource optimization and {SFC} requests in cloud
  datacenter,'' \emph{IEEE Transactions on Parallel and Distributed Systems},
  vol.~29, no.~7, pp. 1664--1677, July 2018.

\bibitem{8501940}
X.~{Chen}, W.~{Ni}, I.~B. {Collings}, X.~{Wang}, and S.~{Xu}, ``Automated
  function placement and online optimization of network functions
  virtualization,'' \emph{IEEE Transactions on Communications}, vol.~67, no.~2,
  pp. 1225--1237, Feb. 2019.

\bibitem{7859379}
C.~{Pham}, N.~H. {Tran}, S.~{Ren}, W.~{Saad}, and C.~S. {Hong}, ``Traffic-aware
  and energy-efficient {VNF} placement for service chaining: Joint sampling and
  matching approach,'' \emph{IEEE Transactions on Services Computing}, pp.
  1--1, 2017.

\bibitem{nejad2018vspace}
M.~A.~T. Nejad, S.~Parsaeefard, M.~A. Maddah-Ali, T.~Mahmoodi, and B.~H.
  Khalaj, ``{vSPACE}: {VNF} simultaneous placement, admission control and
  embedding,'' \emph{IEEE Journal on Selected Areas in Communications},
  vol.~36, no.~3, pp. 542--557, Mar. 2018.

\bibitem{9000731}
J.~{Chen}, H.~{Liu}, and H.~{Jia}, ``Cross-layer resource allocation in
  wireless-enabled {NFV},'' \emph{IEEE Wireless Communications Letters}, pp.
  1--1, IEEE Early Access, Feb. 2020.

\bibitem{7490404}
L.~{Qu}, C.~{Assi}, and K.~{Shaban}, ``Delay-aware scheduling and resource
  optimization with network function virtualization,'' \emph{IEEE Transactions
  on Communications}, vol.~64, no.~9, pp. 3746--3758, Sep. 2016.

\bibitem{game-theroy}
C.~{Pham}, N.~H. {Tran}, and C.~S. {Hong}, ``Virtual network function
  scheduling: A matching game approach,'' \emph{IEEE Communications Letters},
  vol.~22, no.~1, Jan. 2018.

\bibitem{8256017}
H.~A. {Alameddine}, L.~{Qu}, and C.~{Assi}, ``Scheduling service function
  chains for ultra-low latency network services,'' in \emph{2017 13th
  International Conference on Network and Service Management (CNSM)}, 2017, pp.
  1--9.

\bibitem{kim2018performance}
H.~Kim, ``Performance evaluation of revised virtual resources allocation scheme
  in network function virtualization ({NFV}) networks,'' \emph{Cluster
  Computing}, vol.~22, no.~1, pp. 2331--2339, 2019.

\bibitem{8951149}
S.~{Khan Tayyaba}, H.~A. {Khattak}, A.~{Almogren}, M.~A. {Shah}, I.~{Ud Din},
  I.~{Alkhalifa}, and M.~{Guizani}, ``{5G} vehicular network resource
  management for improving radio access through machine learning,'' \emph{IEEE
  Access}, vol.~8, pp. 6792--6800, 2020.

\bibitem{9128963}
J.~{Chen}, J.~{Chen}, R.~{Hu}, and H.~{Zhang}, ``{QMORA}: A {Q-Learning} based
  multi-objective resource allocation scheme for {NFV} orchestration,'' in
  \emph{2020 IEEE 91st Vehicular Technology Conference (VTC2020-Spring)}, 2020,
  pp. 1--6.

\bibitem{8855889}
J.~{Li}, W.~{Shi}, N.~{Zhang}, and X.~S. {Shen}, ``Reinforcement learning based
  {VNF} scheduling with {End-to-End} delay guarantee,'' in \emph{2019 IEEE/CIC
  International Conference on Communications in China (ICCC)}, 2019, pp.
  572--577.

\bibitem{8901169}
S.~{Troia}, R.~{Alvizu}, and G.~{Maier}, ``Reinforcement learning for service
  function chain reconfiguration in {NFV-SDN} metro-core optical networks,''
  \emph{IEEE Access}, vol.~7, pp. 167\,944--167\,957, 2019.

\bibitem{SOFT}
T.~Haarnoja, A.~Zhou, P.~Abbeel, and S.~Levine, ``Soft actor-critic: Off-policy
  maximum entropy deep reinforcement learning with a stochastic actor,'' in
  \emph{International Conference on Machine Learning}.\hskip 1em plus 0.5em
  minus 0.4em\relax PMLR, 2018, pp. 1861--1870.

\bibitem{7949048}
N.~{Yu}, Z.~{Song}, H.~{Du}, H.~{Huang}, and X.~{Jia}, ``Dynamic resource
  provisioning for energy efficient cloud radio access networks,'' \emph{IEEE
  Transactions on Cloud Computing}, vol.~7, no.~4, pp. 964--974, Oct. 2019.

\bibitem{ETSIG003}
{ETSI, GSNFV}, ``Network functions virtualisation ({NFV}); terminology for main
  concepts in {NFV},'' \emph{ETSI GS NFV}, vol.~2, no.~2, p.~V1, Aug. 2018.

\bibitem{etsi2013network}
------, ``Network functions virtualisation ({NFV}): Architectural framework,''
  \emph{ETSI GS NFV}, vol.~2, no.~2, p.~V1, 2018.

\bibitem{yoon2016nfv}
M.~S. Yoon and A.~E. Kamal, ``{NFV} resource allocation using mixed queuing
  network model,'' in \emph{in Proc. IEEE Global Communications Conference
  (GLOBECOM)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2016, pp.
  Washington, DC, USA, 1--6. Dec. 2016.

\bibitem{9076109}
Z.~{Shu} and T.~{Taleb}, ``A novel {QoS} framework for network slicing in {5G}
  and beyond networks based on {SDN} and {NFV},'' \emph{IEEE Network}, vol.~34,
  no.~3, pp. 256--263, 2020.

\bibitem{8423711}
G.~{Sun}, Y.~{Li}, D.~{Liao}, and V.~{Chang}, ``Service function chain
  orchestration across multiple domains: A full mesh aggregation approach,''
  \emph{IEEE Transactions on Network and Service Management}, vol.~15, no.~3,
  pp. 1175--1191, 2018.

\bibitem{7387398}
S.~{Van Rossem}, W.~{Tavernier}, B.~{Sonkoly}, D.~{Colle}, J.~{Czentye},
  M.~{Pickavet}, and P.~{Demeester}, ``Deploying elastic routing capability in
  an {SDN/NFV}-enabled environment,'' in \emph{2015 {IEEE} Conference on
  Network Function Virtualization and Software Defined Network ({NFV-SDN})},
  2015, pp. 22--24.

\bibitem{7279063}
M.~{Dayarathna}, Y.~{Wen}, and R.~{Fan}, ``Data center energy consumption
  modeling: A survey,'' \emph{IEEE Communications Surveys Tutorials}, vol.~18,
  no.~1, pp. 732--794, 2016.

\bibitem{17reinforcement}
T.~Haarnoja, H.~Tang, P.~Abbeel, and S.~Levine, ``Reinforcement learning with
  deep energy-based policies,'' in \emph{International Conference on Machine
  Learning}.\hskip 1em plus 0.5em minus 0.4em\relax PMLR, 2017, pp. 1352--1361.

\bibitem{conventional}
C.~Zhong, Z.~Lu, M.~C. Gursoy, and S.~Velipasalar, ``A deep actor-critic
  reinforcement learning framework for dynamic multichannel access,''
  \emph{IEEE Transactions on Cognitive Communications and Networking}, vol.~5,
  no.~4, pp. 1125--1139, 2019.

\bibitem{sutton2018reinforcement}
R.~S. Sutton and A.~G. Barto, \emph{Reinforcement learning: An
  introduction}.\hskip 1em plus 0.5em minus 0.4em\relax MIT press, 2018.

\bibitem{SoAcCrDRL}
F.~Fu, Y.~Kang, Z.~Zhang, F.~R. Yu, and T.~Wu, ``Soft actor–critic {DRL} for
  live transcoding and streaming in vehicular {Fog}-computing-enabled {IoV},''
  \emph{IEEE Internet of Things Journal}, vol.~8, no.~3, pp. 1308--1321, 2021.

\bibitem{817021999}
Z.~{Li} and C.~{Guo}, ``Multi-agent deep reinforcement learning based spectrum
  allocation for {D2D} underlay communications,'' \emph{IEEE Transactions on
  Vehicular Technology}, vol.~69, no.~2, pp. 1828--1840, 2020.

\bibitem{grondman2012survey}
I.~Grondman, L.~Busoniu, G.~A. Lopes, and R.~Babuska, ``A survey of
  actor-critic reinforcement learning: Standard and natural policy gradients,''
  \emph{IEEE Transactions on Systems, Man, and Cybernetics, Part C
  (Applications and Reviews)}, vol.~42, no.~6, pp. 1291--1307, 2012.

\bibitem{817021888}
C.~J. {Watkins} and P.~{Dayan}, ``Q-learning,'' \emph{Machine Learning},
  vol.~8, no.~4, p. 279–292, 1992.

\bibitem{8170218888}
J.~{Hu}, H.~{Zhang}, L.~{Song}, R.~{Schober}, and H.~V. {Poor}, \emph{IEEE
  Transactions on Communications}.

\bibitem{861130000}
M.~{Savi}, M.~{Tornatore}, and G.~{Verticale}, ``Impact of processing-resource
  sharing on the placement of chained virtual network functions,'' \emph{IEEE
  Transactions on Cloud Computing}, 2019.

\bibitem{ebrahimi2020joint}
S.~Ebrahimi, A.~Zakeri, B.~Akbari, and N.~Mokari, ``Joint resource and
  admission management for slice-enabled networks,'' in \emph{NOMS 2020-2020
  IEEE/IFIP Network Operations and Management Symposium}.\hskip 1em plus 0.5em
  minus 0.4em\relax IEEE, 2020, pp. 1--7.

\bibitem{xiao2019nfvdeep}
Y.~Xiao, Q.~Zhang, F.~Liu, J.~Wang, M.~Zhao, Z.~Zhang, and J.~Zhang, ``Nfvdeep:
  Adaptive online service function chain deployment with deep reinforcement
  learning,'' in \emph{Proceedings of the International Symposium on Quality of
  Service}, 2019, pp. 1--10.

\bibitem{ng2011resource}
D.~W.~K. Ng and R.~Schober, ``Resource allocation and scheduling in multi-cell
  ofdma systems with decode-and-forward relaying,'' \emph{IEEE Transactions on
  Wireless Communications}, vol.~10, no.~7, pp. 2246--2258, 2011.

\end{thebibliography}

